Modular knots obey the Chebotarev law for compact Lie groups

The modular knots are the closed orbits of the geodesic flow on the complement of a trefoil in $S^{3}$. McMullen proved that the closed orbits of a mixing pseudo-Anosov flow on a closed $3$-manifold obey the Chebotarev law for a compact Lie group whose identity component is semisimple. For the modular knots ordered by the trace, we remove the assumption on the group: the cusp, along which the linking numbers grow linearly while the hyperbolic lengths grow logarithmically, prevents any character from being a function of the length. For the generic and for the combinatorial ordering we determine the exceptions: by the criterion of Parry and Pollicott, the law fails exactly for the characters that are functions of the length, and then the Frobenius classes are still equidistributed in the fibers over the torus of these characters and in logarithmic density. For $\mathrm{SU}(2)$ the traces obey the Sato--Tate law.

==> mkc1_labels.tex <==
\makeatletter
\expandafter\def\csname PI@sec.intro\endcsname{Section~1}\expandafter\def\csname PIn@sec.intro\endcsname{1}
\expandafter\def\csname PI@subsec.intro.law\endcsname{Section~1.1}\expandafter\def\csname PIn@subsec.intro.law\endcsname{1.1}
\expandafter\def\csname PI@dfn.Chebotarev\endcsname{Definition~1.1}\expandafter\def\csname PIn@dfn.Chebotarev\endcsname{1.1}
\expandafter\def\csname PI@table.orderings\endcsname{Table~1}\expandafter\def\csname PIn@table.orderings\endcsname{1}
\expandafter\def\csname PI@subsec.intro.results\endcsname{Section~1.2}\expandafter\def\csname PIn@subsec.intro.results\endcsname{1.2}
\expandafter\def\csname PI@thmA.combinatorial\endcsname{Theorem~A}\expandafter\def\csname PIn@thmA.combinatorial\endcsname{A}
\expandafter\def\csname PI@thmA.generic\endcsname{Theorem~B}\expandafter\def\csname PIn@thmA.generic\endcsname{B}
\expandafter\def\csname PI@thmA.arith\endcsname{Theorem~C}\expandafter\def\csname PIn@thmA.arith\endcsname{C}
\expandafter\def\csname PI@thmA.densities\endcsname{Theorem~D}\expandafter\def\csname PIn@thmA.densities\endcsname{D}
\expandafter\def\csname PI@corA.linking\endcsname{Corollary~E}\expandafter\def\csname PIn@corA.linking\endcsname{E}
\expandafter\def\csname PI@subsec.intro.branched\endcsname{Section~1.3}\expandafter\def\csname PIn@subsec.intro.branched\endcsname{1.3}
\expandafter\def\csname PI@thmA.branched\endcsname{Theorem~F}\expandafter\def\csname PIn@thmA.branched\endcsname{F}
\expandafter\def\csname PI@thmA.finiteindex\endcsname{Theorem~G}\expandafter\def\csname PIn@thmA.finiteindex\endcsname{G}
\expandafter\def\csname PI@subsec.intro.compact\endcsname{Section~1.4}\expandafter\def\csname PIn@subsec.intro.compact\endcsname{1.4}
\expandafter\def\csname PI@subsec.intro.method\endcsname{Section~1.5}\expandafter\def\csname PIn@subsec.intro.method\endcsname{1.5}
\expandafter\def\csname PI@subsec.intro.plan\endcsname{Section~1.6}\expandafter\def\csname PIn@subsec.intro.plan\endcsname{1.6}
\expandafter\def\csname PI@sec.background\endcsname{Section~2}\expandafter\def\csname PIn@sec.background\endcsname{2}
\expandafter\def\csname PI@subsec.bg.modular\endcsname{Section~2.1}\expandafter\def\csname PIn@subsec.bg.modular\endcsname{2.1}
\expandafter\def\csname PI@subsec.bg.rademacher\endcsname{Section~2.2}\expandafter\def\csname PIn@subsec.bg.rademacher\endcsname{2.2}
\expandafter\def\csname PI@thm.ghys\endcsname{Theorem~2.1}\expandafter\def\csname PIn@thm.ghys\endcsname{2.1}
\expandafter\def\csname PI@subsec.bg.lorenz\endcsname{Section~2.3}\expandafter\def\csname PIn@subsec.bg.lorenz\endcsname{2.3}
\expandafter\def\csname PI@subsec.bg.distribution\endcsname{Section~2.4}\expandafter\def\csname PIn@subsec.bg.distribution\endcsname{2.4}
\expandafter\def\csname PI@thm.cauchy\endcsname{Theorem~2.2}\expandafter\def\csname PIn@thm.cauchy\endcsname{2.2}
\expandafter\def\csname PI@sec.ordering\endcsname{Section~3}\expandafter\def\csname PIn@sec.ordering\endcsname{3}
\expandafter\def\csname PI@subsec.ord.roof\endcsname{Section~3.1}\expandafter\def\csname PIn@subsec.ord.roof\endcsname{3.1}
\expandafter\def\csname PI@subsec.ord.compare\endcsname{Section~3.2}\expandafter\def\csname PIn@subsec.ord.compare\endcsname{3.2}
\expandafter\def\csname PI@prop.incommensurable\endcsname{Proposition~3.1}\expandafter\def\csname PIn@prop.incommensurable\endcsname{3.1}
\expandafter\def\csname PI@rem.crossings\endcsname{Remark~3.2}\expandafter\def\csname PIn@rem.crossings\endcsname{3.2}
\expandafter\def\csname PI@subsec.ord.laws\endcsname{Section~3.3}\expandafter\def\csname PIn@subsec.ord.laws\endcsname{3.3}
\expandafter\def\csname PI@thm.two.densities\endcsname{Theorem~3.3}\expandafter\def\csname PIn@thm.two.densities\endcsname{3.3}
\expandafter\def\csname PI@rem.densities.numerics\endcsname{Remark~3.4}\expandafter\def\csname PIn@rem.densities.numerics\endcsname{3.4}
\expandafter\def\csname PI@prop.density.ellh\endcsname{Proposition~3.5}\expandafter\def\csname PIn@prop.density.ellh\endcsname{3.5}
\expandafter\def\csname PI@rem.exact.length\endcsname{Remark~3.6}\expandafter\def\csname PIn@rem.exact.length\endcsname{3.6}
\expandafter\def\csname PI@cor.three.densities\endcsname{Corollary~3.7}\expandafter\def\csname PIn@cor.three.densities\endcsname{3.7}
\expandafter\def\csname PI@sec.symbolic\endcsname{Section~4}\expandafter\def\csname PIn@sec.symbolic\endcsname{4}
\expandafter\def\csname PI@subsec.graph\endcsname{Section~4.1}\expandafter\def\csname PIn@subsec.graph\endcsname{4.1}
\expandafter\def\csname PI@lem.irreducible\endcsname{Lemma~4.1}\expandafter\def\csname PIn@lem.irreducible\endcsname{4.1}
\expandafter\def\csname PI@rem.dense.orbit\endcsname{Remark~4.2}\expandafter\def\csname PIn@rem.dense.orbit\endcsname{4.2}
\expandafter\def\csname PI@subsec.suspension\endcsname{Section~4.2}\expandafter\def\csname PIn@subsec.suspension\endcsname{4.2}
\expandafter\def\csname PI@subsec.mixing\endcsname{Section~4.3}\expandafter\def\csname PIn@subsec.mixing\endcsname{4.3}
\expandafter\def\csname PI@eq.circle\endcsname{(4.1)}\expandafter\def\csname PIn@eq.circle\endcsname{4.1}
\expandafter\def\csname PI@subsec.frobenius\endcsname{Section~4.4}\expandafter\def\csname PIn@subsec.frobenius\endcsname{4.4}
\expandafter\def\csname PI@dfn.frobenius\endcsname{Definition~4.3}\expandafter\def\csname PIn@dfn.frobenius\endcsname{4.3}
\expandafter\def\csname PI@rem.PP.convention\endcsname{Remark~4.4}\expandafter\def\csname PIn@rem.PP.convention\endcsname{4.4}
\expandafter\def\csname PI@subsec.PP\endcsname{Section~4.5}\expandafter\def\csname PIn@subsec.PP\endcsname{4.5}
\expandafter\def\csname PI@thm.PP\endcsname{Theorem~4.5}\expandafter\def\csname PIn@thm.PP\endcsname{4.5}
\expandafter\def\csname PI@lem.ties\endcsname{Lemma~4.6}\expandafter\def\csname PIn@lem.ties\endcsname{4.6}
\expandafter\def\csname PI@cor.nocircle\endcsname{Corollary~4.7}\expandafter\def\csname PIn@cor.nocircle\endcsname{4.7}
\expandafter\def\csname PI@lem.finitely.many\endcsname{Lemma~4.8}\expandafter\def\csname PIn@lem.finitely.many\endcsname{4.8}
\expandafter\def\csname PI@sec.flat\endcsname{Section~5}\expandafter\def\csname PIn@sec.flat\endcsname{5}
\expandafter\def\csname PI@lem.dense\endcsname{Lemma~5.1}\expandafter\def\csname PIn@lem.dense\endcsname{5.1}
\expandafter\def\csname PI@thm.flat\endcsname{Theorem~5.2}\expandafter\def\csname PIn@thm.flat\endcsname{5.2}
\expandafter\def\csname PI@rem.flat.finite\endcsname{Remark~5.3}\expandafter\def\csname PIn@rem.flat.finite\endcsname{5.3}
\expandafter\def\csname PI@sec.markov\endcsname{Section~6}\expandafter\def\csname PIn@sec.markov\endcsname{6}
\expandafter\def\csname PI@subsec.rectangle\endcsname{Section~6.1}\expandafter\def\csname PIn@subsec.rectangle\endcsname{6.1}
\expandafter\def\csname PI@subsec.markov.cond\endcsname{Section~6.2}\expandafter\def\csname PIn@subsec.markov.cond\endcsname{6.2}
\expandafter\def\csname PI@dfn.markov\endcsname{Definition~6.1}\expandafter\def\csname PIn@dfn.markov\endcsname{6.1}
\expandafter\def\csname PI@rem.bounded\endcsname{Remark~6.2}\expandafter\def\csname PIn@rem.bounded\endcsname{6.2}
\expandafter\def\csname PI@subsec.coding\endcsname{Section~6.3}\expandafter\def\csname PIn@subsec.coding\endcsname{6.3}
\expandafter\def\csname PI@lem.arcs\endcsname{Lemma~6.3}\expandafter\def\csname PIn@lem.arcs\endcsname{6.3}
\expandafter\def\csname PI@lem.orbits.bijection\endcsname{Lemma~6.4}\expandafter\def\csname PIn@lem.orbits.bijection\endcsname{6.4}
\expandafter\def\csname PI@subsec.irreducible\endcsname{Section~6.4}\expandafter\def\csname PIn@subsec.irreducible\endcsname{6.4}
\expandafter\def\csname PI@lem.flow.irreducible\endcsname{Lemma~6.5}\expandafter\def\csname PIn@lem.flow.irreducible\endcsname{6.5}
\expandafter\def\csname PI@sec.spine\endcsname{Section~7}\expandafter\def\csname PIn@sec.spine\endcsname{7}
\expandafter\def\csname PI@subsec.boxes\endcsname{Section~7.1}\expandafter\def\csname PIn@subsec.boxes\endcsname{7.1}
\expandafter\def\csname PI@rem.contractible\endcsname{Remark~7.1}\expandafter\def\csname PIn@rem.contractible\endcsname{7.1}
\expandafter\def\csname PI@lem.VU\endcsname{Lemma~7.2}\expandafter\def\csname PIn@lem.VU\endcsname{7.2}
\expandafter\def\csname PI@lem.homotopic\endcsname{Lemma~7.3}\expandafter\def\csname PIn@lem.homotopic\endcsname{7.3}
\expandafter\def\csname PI@subsec.surj\endcsname{Section~7.2}\expandafter\def\csname PIn@subsec.surj\endcsname{7.2}
\expandafter\def\csname PI@lem.surj\endcsname{Lemma~7.4}\expandafter\def\csname PIn@lem.surj\endcsname{7.4}
\expandafter\def\csname PI@fig.deformation\endcsname{Figure~1}\expandafter\def\csname PIn@fig.deformation\endcsname{1}
\expandafter\def\csname PI@rem.dichotomy\endcsname{Remark~7.5}\expandafter\def\csname PIn@rem.dichotomy\endcsname{7.5}
\expandafter\def\csname PI@sec.escape\endcsname{Section~8}\expandafter\def\csname PIn@sec.escape\endcsname{8}
\expandafter\def\csname PI@thm.main.general\endcsname{Theorem~8.1}\expandafter\def\csname PIn@thm.main.general\endcsname{8.1}
\expandafter\def\csname PI@lem.refinement.markov\endcsname{Lemma~8.2}\expandafter\def\csname PIn@lem.refinement.markov\endcsname{8.2}
\expandafter\def\csname PI@fig.refinement\endcsname{Figure~2}\expandafter\def\csname PIn@fig.refinement\endcsname{2}
\expandafter\def\csname PI@lem.refined.nonarithmetic\endcsname{Lemma~8.3}\expandafter\def\csname PIn@lem.refined.nonarithmetic\endcsname{8.3}
\expandafter\def\csname PI@lem.infinitely.many\endcsname{Lemma~8.4}\expandafter\def\csname PIn@lem.infinitely.many\endcsname{8.4}
\expandafter\def\csname PI@sec.modular\endcsname{Section~9}\expandafter\def\csname PIn@sec.modular\endcsname{9}
\expandafter\def\csname PI@subsec.farey\endcsname{Section~9.1}\expandafter\def\csname PIn@subsec.farey\endcsname{9.1}
\expandafter\def\csname PI@prop.modular\endcsname{Proposition~9.1}\expandafter\def\csname PIn@prop.modular\endcsname{9.1}
\expandafter\def\csname PI@fig.farey\endcsname{Figure~3}\expandafter\def\csname PIn@fig.farey\endcsname{3}
\expandafter\def\csname PI@subsec.farey.orbits\endcsname{Section~9.2}\expandafter\def\csname PIn@subsec.farey.orbits\endcsname{9.2}
\expandafter\def\csname PI@fig.horseshoe\endcsname{Figure~4}\expandafter\def\csname PIn@fig.horseshoe\endcsname{4}
\expandafter\def\csname PI@lem.tails\endcsname{Lemma~9.2}\expandafter\def\csname PIn@lem.tails\endcsname{9.2}
\expandafter\def\csname PI@subsec.four\endcsname{Section~9.3}\expandafter\def\csname PIn@subsec.four\endcsname{9.3}
\expandafter\def\csname PI@prop.modular.four\endcsname{Proposition~9.3}\expandafter\def\csname PIn@prop.modular.four\endcsname{9.3}
\expandafter\def\csname PI@subsec.induced\endcsname{Section~9.4}\expandafter\def\csname PIn@subsec.induced\endcsname{9.4}
\expandafter\def\csname PI@prop.induced\endcsname{Proposition~9.4}\expandafter\def\csname PIn@prop.induced\endcsname{9.4}
\expandafter\def\csname PI@fig.induced\endcsname{Figure~5}\expandafter\def\csname PIn@fig.induced\endcsname{5}
\expandafter\def\csname PI@rem.modular.sources\endcsname{Remark~9.5}\expandafter\def\csname PIn@rem.modular.sources\endcsname{9.5}
\expandafter\def\csname PI@subsec.refine\endcsname{Section~9.5}\expandafter\def\csname PIn@subsec.refine\endcsname{9.5}
\expandafter\def\csname PI@prop.refine\endcsname{Proposition~9.6}\expandafter\def\csname PIn@prop.refine\endcsname{9.6}
\expandafter\def\csname PI@lem.refine.realized\endcsname{Lemma~9.7}\expandafter\def\csname PIn@lem.refine.realized\endcsname{9.7}
\expandafter\def\csname PI@subsec.modular.generic\endcsname{Section~9.6}\expandafter\def\csname PIn@subsec.modular.generic\endcsname{9.6}
\expandafter\def\csname PI@thm.modular\endcsname{Theorem~9.8}\expandafter\def\csname PIn@thm.modular\endcsname{9.8}
\expandafter\def\csname PI@eg.explicit.ordering\endcsname{Example~9.9}\expandafter\def\csname PIn@eg.explicit.ordering\endcsname{9.9}
\expandafter\def\csname PI@subsec.cusp\endcsname{Section~9.7}\expandafter\def\csname PIn@subsec.cusp\endcsname{9.7}
\expandafter\def\csname PI@prop.no.finite.markov\endcsname{Proposition~9.10}\expandafter\def\csname PIn@prop.no.finite.markov\endcsname{9.10}
\expandafter\def\csname PI@prop.not.closed.orbit\endcsname{Proposition~9.11}\expandafter\def\csname PIn@prop.not.closed.orbit\endcsname{9.11}
\expandafter\def\csname PI@eq.one.direction\endcsname{(9.1)}\expandafter\def\csname PIn@eq.one.direction\endcsname{9.1}
\expandafter\def\csname PI@cor.not.closed.orbit\endcsname{Corollary~9.12}\expandafter\def\csname PIn@cor.not.closed.orbit\endcsname{9.12}
\expandafter\def\csname PI@q.time.change\endcsname{Question~9.13}\expandafter\def\csname PIn@q.time.change\endcsname{9.13}
\expandafter\def\csname PI@prop.no.completion\endcsname{Proposition~9.14}\expandafter\def\csname PIn@prop.no.completion\endcsname{9.14}
\expandafter\def\csname PI@sec.combinatorial\endcsname{Section~10}\expandafter\def\csname PIn@sec.combinatorial\endcsname{10}
\expandafter\def\csname PI@eq.simon\endcsname{(10.1)}\expandafter\def\csname PIn@eq.simon\endcsname{10.1}
\expandafter\def\csname PI@lem.link.cusp\endcsname{Lemma~10.1}\expandafter\def\csname PIn@lem.link.cusp\endcsname{10.1}
\expandafter\def\csname PI@eq.trace\endcsname{(10.2)}\expandafter\def\csname PIn@eq.trace\endcsname{10.2}
\expandafter\def\csname PI@lem.twisted\endcsname{Lemma~10.2}\expandafter\def\csname PIn@lem.twisted\endcsname{10.2}
\expandafter\def\csname PI@eq.section\endcsname{(10.3)}\expandafter\def\csname PIn@eq.section\endcsname{10.3}
\expandafter\def\csname PI@thm.combinatorial\endcsname{Theorem~10.3}\expandafter\def\csname PIn@thm.combinatorial\endcsname{10.3}
\expandafter\def\csname PI@eq.primitive.count\endcsname{(10.4)}\expandafter\def\csname PIn@eq.primitive.count\endcsname{10.4}
\expandafter\def\csname PI@eq.count.twisted\endcsname{(10.5)}\expandafter\def\csname PIn@eq.count.twisted\endcsname{10.5}
\expandafter\def\csname PI@eq.Pn\endcsname{(10.6)}\expandafter\def\csname PIn@eq.Pn\endcsname{10.6}
\expandafter\def\csname PI@eq.special\endcsname{(10.7)}\expandafter\def\csname PIn@eq.special\endcsname{10.7}
\expandafter\def\csname PI@eq.character\endcsname{(10.8)}\expandafter\def\csname PIn@eq.character\endcsname{10.8}
\expandafter\def\csname PI@eq.remaining\endcsname{(10.9)}\expandafter\def\csname PIn@eq.remaining\endcsname{10.9}
\expandafter\def\csname PI@cor.combinatorial\endcsname{Corollary~10.4}\expandafter\def\csname PIn@cor.combinatorial\endcsname{10.4}
\expandafter\def\csname PI@rem.combinatorial.ties\endcsname{Remark~10.5}\expandafter\def\csname PIn@rem.combinatorial.ties\endcsname{10.5}
\expandafter\def\csname PI@sec.arith\endcsname{Section~11}\expandafter\def\csname PIn@sec.arith\endcsname{11}
\expandafter\def\csname PI@subsec.transfer\endcsname{Section~11.1}\expandafter\def\csname PIn@subsec.transfer\endcsname{11.1}
\expandafter\def\csname PI@lem.nuclear\endcsname{Lemma~11.1}\expandafter\def\csname PIn@lem.nuclear\endcsname{11.1}
\expandafter\def\csname PI@subsec.fredholm\endcsname{Section~11.2}\expandafter\def\csname PIn@subsec.fredholm\endcsname{11.2}
\expandafter\def\csname PI@prop.fredholm\endcsname{Proposition~11.2}\expandafter\def\csname PIn@prop.fredholm\endcsname{11.2}
\expandafter\def\csname PI@subsec.non-vanishing\endcsname{Section~11.3}\expandafter\def\csname PIn@subsec.non-vanishing\endcsname{11.3}
\expandafter\def\csname PI@lem.non-vanishing\endcsname{Lemma~11.3}\expandafter\def\csname PIn@lem.non-vanishing\endcsname{11.3}
\expandafter\def\csname PI@eq.domination\endcsname{(11.1)}\expandafter\def\csname PIn@eq.domination\endcsname{11.1}
\expandafter\def\csname PI@eq.cohom\endcsname{(11.2)}\expandafter\def\csname PIn@eq.cohom\endcsname{11.2}
\expandafter\def\csname PI@rem.numerics\endcsname{Remark~11.4}\expandafter\def\csname PIn@rem.numerics\endcsname{11.4}
\expandafter\def\csname PI@subsec.tauberian\endcsname{Section~11.4}\expandafter\def\csname PIn@subsec.tauberian\endcsname{11.4}
\expandafter\def\csname PI@lem.hol\endcsname{Lemma~11.5}\expandafter\def\csname PIn@lem.hol\endcsname{11.5}
\expandafter\def\csname PI@thm.arith\endcsname{Theorem~11.6}\expandafter\def\csname PIn@thm.arith\endcsname{11.6}
\expandafter\def\csname PI@cor.rademacher\endcsname{Corollary~11.7}\expandafter\def\csname PIn@cor.rademacher\endcsname{11.7}
\expandafter\def\csname PI@subsec.arith.removing\endcsname{Section~11.5}\expandafter\def\csname PIn@subsec.arith.removing\endcsname{11.5}
\expandafter\def\csname PI@thm.arith.general\endcsname{Theorem~11.8}\expandafter\def\csname PIn@thm.arith.general\endcsname{11.8}
\expandafter\def\csname PI@rem.burrin.vonessen\endcsname{Remark~11.9}\expandafter\def\csname PIn@rem.burrin.vonessen\endcsname{11.9}
\expandafter\def\csname PI@rem.arith.sources\endcsname{Remark~11.10}\expandafter\def\csname PIn@rem.arith.sources\endcsname{11.10}
\expandafter\def\csname PI@sec.linking\endcsname{Section~12}\expandafter\def\csname PIn@sec.linking\endcsname{12}
\expandafter\def\csname PI@cor.linking\endcsname{Corollary~12.1}\expandafter\def\csname PIn@cor.linking\endcsname{12.1}
\expandafter\def\csname PI@rem.linking.joint\endcsname{Remark~12.2}\expandafter\def\csname PIn@rem.linking.joint\endcsname{12.2}
\expandafter\def\csname PI@cor.two.symbols\endcsname{Corollary~12.3}\expandafter\def\csname PIn@cor.two.symbols\endcsname{12.3}
\expandafter\def\csname PI@rem.two.symbols\endcsname{Remark~12.4}\expandafter\def\csname PIn@rem.two.symbols\endcsname{12.4}
\expandafter\def\csname PI@sec.stably.chebotarev\endcsname{Section~13}\expandafter\def\csname PIn@sec.stably.chebotarev\endcsname{13}
\expandafter\def\csname PI@subsec.branched.general\endcsname{Section~13.1}\expandafter\def\csname PIn@subsec.branched.general\endcsname{13.1}
\expandafter\def\csname PI@thm.branched.general\endcsname{Theorem~13.1}\expandafter\def\csname PIn@thm.branched.general\endcsname{13.1}
\expandafter\def\csname PI@subsec.branched.modular\endcsname{Section~13.2}\expandafter\def\csname PIn@subsec.branched.modular\endcsname{13.2}
\expandafter\def\csname PI@thm.branched\endcsname{Theorem~13.2}\expandafter\def\csname PIn@thm.branched\endcsname{13.2}
\expandafter\def\csname PI@sec.finiteindex\endcsname{Section~14}\expandafter\def\csname PIn@sec.finiteindex\endcsname{14}
\expandafter\def\csname PI@thm.finiteindex\endcsname{Theorem~14.1}\expandafter\def\csname PIn@thm.finiteindex\endcsname{14.1}
\expandafter\def\csname PI@sec.remarks\endcsname{Section~15}\expandafter\def\csname PIn@sec.remarks\endcsname{15}
\expandafter\def\csname PI@subsec.rem.icft\endcsname{Section~15.1}\expandafter\def\csname PIn@subsec.rem.icft\endcsname{15.1}
\expandafter\def\csname PI@subsec.rem.supersingular\endcsname{Section~15.2}\expandafter\def\csname PIn@subsec.rem.supersingular\endcsname{15.2}
\expandafter\def\csname PI@subsec.rem.NU\endcsname{Section~15.3}\expandafter\def\csname PIn@subsec.rem.NU\endcsname{15.3}
\expandafter\def\csname PI@subsec.rem.questions\endcsname{Section~15.4}\expandafter\def\csname PIn@subsec.rem.questions\endcsname{15.4}
\expandafter\def\csname PI@subsubsec.q.bias\endcsname{Section~15.4.1}\expandafter\def\csname PIn@subsubsec.q.bias\endcsname{15.4.1}
\expandafter\def\csname PI@subsubsec.q.pairs\endcsname{Section~15.4.2}\expandafter\def\csname PIn@subsubsec.q.pairs\endcsname{15.4.2}
\expandafter\def\csname PI@subsubsec.q.lfunctions\endcsname{Section~15.4.3}\expandafter\def\csname PIn@subsubsec.q.lfunctions\endcsname{15.4.3}
\makeatother

